A Cross-Platform Benchmark for Interval Computation Libraries

Interval computation is widely used to certify computations that use floating point operations to avoid pitfalls related to rounding error introduced by inaccurate operations. Despite its popularity and practical benefits, support for interval arithmetic is not standardized nor available in mainstream programming languages. We propose the first benchmark for interval computations, coupled with reference solutions computed with exact arithmetic, and compare popular C and C++ libraries over different architectures, operating systems, and compilers. The benchmark allows identifying limitations in existing implementations, and provides a reliable guide on which library to use on each system. We believe that our benchmark will be useful for developers of future interval libraries, as a way to test the correctness and performance of their algorithms.

==> tables/mac_performance.tex <==
\begin{adjustbox}{width=.8\textwidth}
\begin{tabular}{lrrrrr}
\toprule
{} &   FILIB C &    BOOST &   NATIVE SWITCHED &   MULTIPLICATIVE &   PRED SUCC \\
\midrule
 ADDITION                 &     81.97 &   112.41 &                    27.33 &                    \hl{\textbf{9.64}} &              10.79 \\
 SUBTRACTION              &     87.33 &   118.70 &                    29.06 &                   \hl{\textbf{10.15}} &              15.47 \\
 MULTIPLICATION           &     89.57 &   119.43 &                    33.79 &                   35.54 &              \hl{\textbf{33.43}} \\
 DIVISION                 &     81.60 &   117.71 &                    42.53 &                   \hl{\textbf{40.35}} &              42.97 \\
 SQUARE ROOT              &     89.63 &   109.22 &                    34.96 &                   37.63 &              \hl{\textbf{34.77}} \\
 EXPONENTIAL              &    159.57 &   198.69 &                   157.81 &                  157.63 &             \hl{\textbf{157.11}} \\
 SIN                      &    177.83 &   812.14 &                   177.44 &                  177.64 &             \hl{\textbf{176.80}} \\
 COS                      &    172.32 &   733.84 &                   \hl{\textbf{170.12}} &                  170.74 &             171.02 \\
 ARITEMETIC EXPRESSION 1  &    746.72 &  1131.36 &                   383.75 &                  \hl{\textbf{358.03}} &             545.20 \\
 ARITEMETIC EXPRESSION 2  &   1148.74 &  1585.20 &                   515.95 &                  \hl{\textbf{375.67}} &             560.50 \\
 ARITEMETIC EXPRESSION 3  &   1491.85 &  2127.44 &                   765.73 &                  \hl{\textbf{610.75}} &             853.82 \\
 ARITEMETIC EXPRESSION 4  &   3215.92 &  4451.83 &                  1475.67 &                 \hl{\textbf{1010.78}} &            1583.29 \\
 ARITEMETIC EXPRESSION 5  &   2220.97 &  3143.14 &                  1017.08 &                  \hl{\textbf{719.24}} &            1187.19 \\
 ARITEMETIC EXPRESSION 6  &   1124.73 &  1573.93 &                   493.58 &                  \hl{\textbf{355.23}} &             632.58 \\
 ARITEMETIC EXPRESSION 7  &    708.27 &  1006.73 &                   339.67 &                  \hl{\textbf{236.30}} &             396.13 \\
 ARITEMETIC EXPRESSION 8  &    753.20 &  1057.08 &                   346.09 &                  \hl{\textbf{263.89}} &             428.95 \\
 ARITEMETIC EXPRESSION 9  &   3800.00 &  5204.90 &                  1764.86 &                 \hl{\textbf{1241.41}} &            1929.32 \\
 ARITEMETIC EXPRESSION 10 &   1434.39 &  2007.76 &                   663.41 &                  \hl{\textbf{467.27}} &             752.67 \\
 RANDOM EXPRESSION 1      &   2006.60 &  4096.04 &                  1705.95 &                 \hl{\textbf{1639.04}} &            1771.17 \\
 RANDOM EXPRESSION 2      &   1143.79 &   943.65 &                  1081.50 &                 1079.73 &            \hl{\textbf{1078.12}} \\
 RANDOM EXPRESSION 3      &   2945.85 &  6003.04 &                  2253.85 &                 \hl{\textbf{2145.04}} &            2345.29 \\
 RANDOM EXPRESSION 4      &   2685.38 &  5492.01 &                  2115.35 &                 \hl{\textbf{2054.73}} &            2238.00 \\
 RANDOM EXPRESSION 5      &   4847.66 & 11432.11 &                  4068.04 &                 \hl{\textbf{3952.91}} &            4264.01 \\
 RANDOM EXPRESSION 6      &   7677.11 & 19478.16 &                  5717.77 &                 \hl{\textbf{5578.44}} &            6080.40 \\
 RANDOM EXPRESSION 7      &   3593.54 &  6840.72 &                  2941.62 &                 \hl{\textbf{2821.85}} &            3031.76 \\
 RANDOM EXPRESSION 8      &   1196.49 &  2783.13 &                  \hl{\textbf{1109.94}} &                 1118.51 &            1195.18 \\
 RANDOM EXPRESSION 9      &   3510.49 &  6596.25 &                  \hl{\textbf{3250.18}} &                 3276.02 &            3353.03 \\
 RANDOM EXPRESSION 10     &   4675.75 & 10722.55 &                  3428.02 &                 \hl{\textbf{3254.32}} &            3575.63 \\
\bottomrule
\end{tabular}
\end{adjustbox}

==> tables/windows_performance.tex <==
\begin{adjustbox}{width=.8\textwidth}
\begin{tabular}{lrrrrr}
\toprule
{} &   FILIB C &     BOOST &   NATIVE SWITCHED &   MULTIPLICATIVE &   PRED SUCC \\
\midrule
 ADDITION                 &    118.72 &    546.98 &            356.70 &            25.30 &       34.12 \\
 SUBTRACTION              &    111.87 &    621.09 &            380.41 &            25.54 &       31.16 \\
 MULTIPLICATION           &    118.93 &   1485.08 &           1193.86 &            34.42 &       48.05 \\
 DIVISION                 &    122.36 &   1253.09 &           1201.56 &            38.31 &       44.22 \\
 SQUARE ROOT              &    117.26 &   1660.51 &             72.95 &            72.91 &       72.75 \\
 EXPONENTIAL              &    171.46 &   1947.03 &            299.94 &           299.72 &      299.76 \\
 SIN                      &    188.45 &   4770.69 &            174.80 &           174.36 &      175.99 \\
 COS                      &    178.63 &   4592.36 &            162.46 &           162.01 &      162.22 \\
 ARITEMETIC EXPRESSION 1  &   1508.25 &  11649.70 &          10822.81 &           362.99 &      580.68 \\
 ARITEMETIC EXPRESSION 2  &   2148.32 &  17888.11 &          14389.02 &           416.59 &      705.39 \\
 ARITEMETIC EXPRESSION 3  &   2785.15 &  23535.36 &          21365.45 &           595.24 &      886.42 \\
 ARITEMETIC EXPRESSION 4  &   6081.16 &  45308.68 &          40043.58 &          1207.91 &     1786.29 \\
 ARITEMETIC EXPRESSION 5  &   4357.70 &  29302.81 &          26596.97 &           824.95 &     1339.25 \\
 ARITEMETIC EXPRESSION 6  &   2190.58 &  15403.22 &          13810.82 &           435.45 &      794.94 \\
 ARITEMETIC EXPRESSION 7  &   1419.16 &  10509.22 &           9411.26 &           280.06 &      486.35 \\
 ARITEMETIC EXPRESSION 8  &   1424.43 &   9790.63 &           9201.90 &           282.01 &      496.65 \\
 ARITEMETIC EXPRESSION 9  &   7318.11 &  51854.46 &          47292.98 &          1448.37 &     2345.76 \\
 ARITEMETIC EXPRESSION 10 &   2885.52 &  17619.61 &          16017.69 &           559.68 &      958.65 \\
 RANDOM EXPRESSION 1      &   3199.79 &  29970.54 &           7603.76 &          2205.62 &     2394.30 \\
 RANDOM EXPRESSION 2      &   1839.43 &   9354.36 &           2160.57 &          2155.33 &     2155.98 \\
 RANDOM EXPRESSION 3      &   4467.75 &  46055.59 &          12311.64 &          2895.57 &     3139.88 \\
 RANDOM EXPRESSION 4      &   4479.75 &  43161.35 &          10294.49 &          2529.57 &     2754.55 \\
 RANDOM EXPRESSION 5      &   7389.14 &  83910.80 &          17901.25 &          4479.94 &     4865.41 \\
 RANDOM EXPRESSION 6      &  11707.14 & 147160.90 &          38231.25 &          6673.79 &     7492.44 \\
 RANDOM EXPRESSION 7      &   5135.11 &  52197.22 &          14490.50 &          4536.11 &     4763.02 \\
 RANDOM EXPRESSION 8      &   1765.18 &  18977.40 &           3910.20 &          1607.20 &     1705.38 \\
 RANDOM EXPRESSION 9      &   5025.71 &  47611.77 &           7506.08 &          4587.96 &     4692.23 \\
 RANDOM EXPRESSION 10     &   6703.45 &  81488.18 &          18459.56 &          3739.06 &     4167.35 \\
\bottomrule
\end{tabular}
\end{adjustbox}
